SoK: Blockchain Decentralization

Blockchain introduces decentralized trust in peer-to-peer networks, advancing security and democratizing systems. Yet, a unified definition for decentralization remains elusive. Our Systematization of Knowledge (SoK) seeks to bridge this gap, emphasizing quantification and methodological coherence. We've formulated a taxonomy defining blockchain decentralization across five facets: consensus, network, governance, wealth, and transaction. Despite the prevalent focus on consensus decentralization, our novel index, based on Shannon entropy, provides comprehensive insights. Moreover, we delve into alternative metrics like the Gini and Nakamoto Coefficients and the Herfindahl-Hirschman Index (HHI), supplemented by an open-source Python tool on GitHub. In terms of methodology, blockchain research has often bypassed stringent scientific methods. By employing descriptive, predictive, and causal methods, our study showcases the potential of structured research in blockchain. Descriptively, we observe a trend of converging decentralization levels over time. Examining DeFi platforms reveals exchange and lending applications as more decentralized than their payment and derivatives counterparts. Predictively, there's a notable correlation between Ether's returns and transaction decentralization in Ether-backed stablecoins. Causally, Ethereum's transition to the EIP-1559 transaction fee model has a profound impact on DeFi transaction decentralization. To conclude, our work outlines directions for blockchain research, emphasizing the delicate balance among decentralization facets, fostering long-term decentralization, and the ties between decentralization, security, privacy, and efficiency. We end by spotlighting challenges in grasping blockchain decentralization intricacies.

==> tables/table12.tex <==
\begin{table}[!htbp] \centering
  \caption{EIP1559 Regression Discontinuity (Dai)}
  \label{tab:12}
  \resizebox{0.5\textwidth}{!}{
\begin{tabular}{@{\extracolsep{5pt}}lccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
& \multicolumn{3}{c}{\textit{Dependent variable: Decentralization Index EMA}} \
\cr \cline{3-4}
\\[-1.8ex] & (1) & (2) & (3) \\
\hline \\[-1.8ex]
 EIP & 49.041$^{**}$ & 40.341$^{*}$ & 25.859$^{}$ \\
  & (23.678) & (19.703) & (21.516) \\
 Day & 9.035$^{***}$ & 9.961$^{***}$ & 10.153$^{***}$ \\
  & (2.830) & (2.380) & (2.359) \\
 EIP\_Day & -9.372$^{***}$ & -9.142$^{***}$ & -11.866$^{***}$ \\
  & (3.049) & (2.521) & (3.012) \\
 TxTfrValAdjUSD & & -0.000$^{}$ & -0.000$^{}$ \\
  & & (0.000) & (0.000) \\
 TxTfrCnt & & 0.009$^{***}$ & 0.007$^{***}$ \\
  & & (0.002) & (0.003) \\
 ROI & & & 10093.969$^{}$ \\
  & & & (11968.170) \\
 VtyDayRet30d & & & 366942.459$^{}$ \\
  & & & (235038.166) \\
 Intercept & 620.415$^{***}$ & 497.169$^{***}$ & 409.672$^{***}$ \\
  & (18.374) & (42.229) & (68.904) \\
\hline \\[-1.8ex]
 Observations & 34 & 34 & 34 \\
 $R^2$ & 0.704 & 0.813 & 0.830 \\
 Adjusted $R^2$ & 0.674 & 0.779 & 0.785 \\
 Residual Std. Error & 33.837(df = 30) & 27.862(df = 28) & 27.508(df = 26)  \\
 F Statistic & 23.769$^{***}$ (df = 3.0; 30.0) & 24.282$^{***}$ (df = 5.0; 28.0) & 18.182$^{***}$ (df = 7.0; 26.0) \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}}

\raggedleft Exponential moving average alpha = 0.1
\end{table}

==> tables/table13.tex <==
\begin{table}[!htbp] \centering
  \caption{EIP1559 Regression Discontinuity (Aave)}
  \label{tab:13}
  \resizebox{0.5\textwidth}{!}{
\begin{tabular}{@{\extracolsep{5pt}}lccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
& \multicolumn{3}{c}{\textit{Dependent variable: Decentralization Index SMA30}} \
\cr \cline{3-4}
\\[-1.8ex] & (1) & (2) & (3) \\
\hline \\[-1.8ex]
 EIP & -120.207$^{***}$ & 50.901$^{***}$ & -117.673$^{***}$ \\
  & (15.575) & (12.795) & (16.783) \\
 Day & -13.652$^{***}$ & -1.350$^{}$ & -16.117$^{***}$ \\
  & (1.861) & (1.546) & (2.569) \\
 EIP\_Day & 8.572$^{***}$ & 7.184$^{***}$ & 9.090$^{***}$ \\
  & (2.006) & (1.637) & (2.151) \\
 TxTfrValAdjUSD & & -0.000$^{}$ & 0.000$^{}$ \\
  & & (0.000) & (0.000) \\
 TxTfrCnt & & 0.003$^{*}$ & -0.007$^{}$ \\
  & & (0.002) & (0.013) \\
 ROI & & & -145.844$^{}$ \\
  & & & (87.719) \\
 VtyDayRet30d & & & -3104.572$^{}$ \\
  & & & (2037.545) \\
 Intercept & 567.076$^{***}$ & 476.318$^{***}$ & 736.525$^{***}$ \\
  & (12.086) & (27.422) & (105.353) \\
\hline \\[-1.8ex]
 Observations & 34 & 34 & 34 \\
 $R^2$ & 0.974 & 0.931 & 0.979 \\
 Adjusted $R^2$ & 0.971 & 0.918 & 0.973 \\
 Residual Std. Error & 22.257(df = 30) & 18.093(df = 28) & 21.422(df = 26)  \\
 F Statistic & 369.651$^{***}$ (df = 3.0; 30.0) & 75.189$^{***}$ (df = 5.0; 28.0) & 171.927$^{***}$ (df = 7.0; 26.0) \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}}
\end{table}

\begin{table}[H] \centering
  \caption{EIP1559 Regression Discontinuity (Aave)}
    \resizebox{0.5\textwidth}{!}{
\begin{tabular}{@{\extracolsep{5pt}}lccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
& \multicolumn{3}{c}{\textit{Dependent variable: Decentralization Index EMA}} \
\cr \cline{3-4}
\\[-1.8ex] & (1) & (2) & (3) \\
\hline \\[-1.8ex]
 EIP & -43.521$^{**}$ & -48.565$^{***}$ & -40.840$^{***}$ \\
  & (16.989) & (12.082) & (12.461) \\
 Day & -9.436$^{***}$ & -6.836$^{***}$ & -9.112$^{***}$ \\
  & (2.030) & (1.510) & (1.907) \\
 EIP\_Day & 7.258$^{***}$ & 5.017$^{***}$ & 5.355$^{***}$ \\
  & (2.188) & (1.597) & (1.597) \\
 TxTfrValAdjUSD & & -0.000$^{**}$ & -0.000$^{**}$ \\
  & & (0.000) & (0.000) \\
 TxTfrCnt & & 0.049$^{***}$ & 0.053$^{***}$ \\
  & & (0.010) & (0.009) \\
 ROI & & & -80.933$^{}$ \\
  & & & (65.130) \\
 VtyDayRet30d & & & -3282.019$^{**}$ \\
  & & & (1512.855) \\
 Intercept & 439.913$^{***}$ & 364.565$^{***}$ & 531.333$^{***}$ \\
  & (13.184) & (16.019) & (78.223) \\
\hline \\[-1.8ex]
 Observations & 34 & 34 & 34 \\
 $R^2$ & 0.880 & 0.945 & 0.955 \\
 Adjusted $R^2$ & 0.868 & 0.936 & 0.943 \\
 Residual Std. Error & 24.279(df = 30) & 16.968(df = 28) & 15.905(df = 26)  \\
 F Statistic & 73.303$^{***}$ (df = 3.0; 30.0) & 96.733$^{***}$ (df = 5.0; 28.0) & 79.470$^{***}$ (df = 7.0; 26.0) \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}}

\raggedleft Exponential moving average alpha = 0.1
\end{table}

==> tables/table14.tex <==
\begin{table}[!htbp] \centering
  \caption{EIP1559 Regression Discontinuity (Compound)}
  \label{tab:14}
    \resizebox{0.5\textwidth}{!}{
\begin{tabular}{@{\extracolsep{5pt}}lccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
& \multicolumn{3}{c}{\textit{Dependent variable: Decentralization Index SMA30}} \
\cr \cline{3-4}
\\[-1.8ex] & (1) & (2) & (3) \\
\hline \\[-1.8ex]
 EIP & -21.591$^{***}$ & 50.901$^{***}$ & -14.097$^{}$ \\
  & (6.610) & (12.795) & (8.290) \\
 Day & -9.729$^{***}$ & -1.350$^{}$ & -12.468$^{***}$ \\
  & (0.790) & (1.546) & (1.831) \\
 EIP\_Day & 7.089$^{***}$ & 7.184$^{***}$ & 9.224$^{***}$ \\
  & (0.851) & (1.637) & (1.613) \\
 TxTfrValAdjUSD & & -0.000$^{}$ & -0.000$^{}$ \\
  & & (0.000) & (0.000) \\
 TxTfrCnt & & 0.003$^{*}$ & 0.004$^{}$ \\
  & & (0.002) & (0.004) \\
 ROI & & & -34.202$^{}$ \\
  & & & (36.627) \\
 VtyDayRet30d & & & -1314.624$^{*}$ \\
  & & & (768.642) \\
 Intercept & 267.238$^{***}$ & 476.318$^{***}$ & 328.709$^{***}$ \\
  & (5.129) & (27.422) & (39.099) \\
\hline \\[-1.8ex]
 Observations & 34 & 34 & 34 \\
 $R^2$ & 0.975 & 0.931 & 0.981 \\
 Adjusted $R^2$ & 0.973 & 0.918 & 0.975 \\
 Residual Std. Error & 9.445(df = 30) & 18.093(df = 28) & 9.010(df = 26)  \\
 F Statistic & 396.338$^{***}$ (df = 3.0; 30.0) & 75.189$^{***}$ (df = 5.0; 28.0) & 187.661$^{***}$ (df = 7.0; 26.0) \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}}
\end{table}

\begin{table}[H] \centering
  \caption{EIP1559 Regression Discontinuity (Compound)}
  \resizebox{0.5\textwidth}{!}{
\begin{tabular}{@{\extracolsep{5pt}}lccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
& \multicolumn{3}{c}{\textit{Dependent variable: Decentralization Index EMA}} \
\cr \cline{3-4}
\\[-1.8ex] & (1) & (2) & (3) \\
\hline \\[-1.8ex]
 EIP & 2.216$^{}$ & 12.855$^{}$ & 19.595$^{}$ \\
  & (10.977) & (12.684) & (14.266) \\
 Day & -8.977$^{***}$ & -9.818$^{***}$ & -12.418$^{***}$ \\
  & (1.312) & (1.447) & (3.151) \\
 EIP\_Day & 7.540$^{***}$ & 8.361$^{***}$ & 10.570$^{***}$ \\
  & (1.414) & (1.569) & (2.777) \\
 TxTfrValAdjUSD & & -0.000$^{}$ & -0.000$^{}$ \\
  & & (0.000) & (0.000) \\
 TxTfrCnt & & 0.009$^{}$ & 0.010$^{}$ \\
  & & (0.006) & (0.006) \\
 ROI & & & 50.285$^{}$ \\
  & & & (63.033) \\
 VtyDayRet30d & & & -1070.005$^{}$ \\
  & & & (1322.778) \\
 Intercept & 217.761$^{***}$ & 200.998$^{***}$ & 249.260$^{***}$ \\
  & (8.518) & (18.566) & (67.286) \\
\hline \\[-1.8ex]
 Observations & 34 & 34 & 34 \\
 $R^2$ & 0.859 & 0.875 & 0.880 \\
 Adjusted $R^2$ & 0.845 & 0.852 & 0.848 \\
 Residual Std. Error & 15.686(df = 30) & 15.287(df = 28) & 15.506(df = 26)  \\
 F Statistic & 60.762$^{***}$ (df = 3.0; 30.0) & 39.105$^{***}$ (df = 5.0; 28.0) & 27.322$^{***}$ (df = 7.0; 26.0) \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}}

\raggedleft Exponential moving average alpha = 0.1
\end{table}

==> tables/table15.tex <==
\begin{table}[!htbp] \centering
  \caption{EIP1559 Regression Discontinuity (Tether)}
  \label{tab:15}
    \resizebox{0.5\textwidth}{!}{
\begin{tabular}{@{\extracolsep{5pt}}lccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
& \multicolumn{3}{c}{\textit{Dependent variable: Decentralization Index SMA30}} \
\cr \cline{3-4}
\\[-1.8ex] & (1) & (2) & (3) \\
\hline \\[-1.8ex]
 EIP & 225.818$^{**}$ & 50.901$^{***}$ & 108.269$^{}$ \\
  & (89.576) & (12.795) & (115.881) \\
 Day & -19.371$^{*}$ & -1.350$^{}$ & -28.141$^{**}$ \\
  & (10.705) & (1.546) & (13.140) \\
 EIP\_Day & 10.434$^{}$ & 7.184$^{***}$ & 5.831$^{}$ \\
  & (11.537) & (1.637) & (12.048) \\
 TxTfrValAdjUSD & & -0.000$^{}$ & 0.000$^{}$ \\
  & & (0.000) & (0.000) \\
 TxTfrCnt & & 0.003$^{*}$ & -0.151$^{}$ \\
  & & (0.002) & (0.135) \\
 ROI & & & -43215.965$^{}$ \\
  & & & (84763.161) \\
 VtyDayRet30d & & & 4149798.180$^{}$ \\
  & & & (2791611.336) \\
 Intercept & 4438.113$^{***}$ & 476.318$^{***}$ & 3647.884$^{***}$ \\
  & (69.511) & (27.422) & (575.175) \\
\hline \\[-1.8ex]
 Observations & 34 & 34 & 34 \\
 $R^2$ & 0.205 & 0.931 & 0.290 \\
 Adjusted $R^2$ & 0.125 & 0.918 & 0.099 \\
 Residual Std. Error & 128.008(df = 30) & 18.093(df = 28) & 129.938(df = 26)  \\
 F Statistic & 2.573$^{*}$ (df = 3.0; 30.0) & 75.189$^{***}$ (df = 5.0; 28.0) & 1.515$^{}$ (df = 7.0; 26.0) \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}}
\end{table}









\begin{table}[H] \centering
  \caption{EIP1559 Regression Discontinuity (Tether)}
    \resizebox{0.5\textwidth}{!}{
\begin{tabular}{@{\extracolsep{5pt}}lccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
& \multicolumn{3}{c}{\textit{Dependent variable: Decentralization Index EMA}} \
\cr \cline{3-4}
\\[-1.8ex] & (1) & (2) & (3) \\
\hline \\[-1.8ex]
 EIP & 569.866$^{***}$ & 549.591$^{***}$ & 253.912$^{}$ \\
  & (171.705) & (175.859) & (210.625) \\
 Day & -26.997$^{}$ & -24.498$^{}$ & -53.780$^{**}$ \\
  & (20.519) & (21.031) & (23.883) \\
 EIP\_Day & -14.376$^{}$ & -14.981$^{}$ & -25.877$^{}$ \\
  & (22.114) & (22.520) & (21.899) \\
 TxTfrValAdjUSD & & 0.000$^{}$ & 0.000$^{}$ \\
  & & (0.000) & (0.000) \\
 TxTfrCnt & & -0.248$^{}$ & -0.376$^{}$ \\
  & & (0.252) & (0.245) \\
 ROI & & & -30744.355$^{}$ \\
  & & & (154065.844) \\
 VtyDayRet30d & & & 11643198.502$^{**}$ \\
  & & & (5074043.394) \\
 Intercept & 4424.165$^{***}$ & 4538.355$^{***}$ & 2175.161$^{**}$ \\
  & (133.243) & (182.579) & (1045.439) \\
\hline \\[-1.8ex]
 Observations & 34 & 34 & 34 \\
 $R^2$ & 0.476 & 0.494 & 0.580 \\
 Adjusted $R^2$ & 0.424 & 0.404 & 0.466 \\
 Residual Std. Error & 245.373(df = 30) & 249.604(df = 28) & 236.176(df = 26)  \\
 F Statistic & 9.096$^{***}$ (df = 3.0; 30.0) & 5.473$^{***}$ (df = 5.0; 28.0) & 5.120$^{***}$ (df = 7.0; 26.0) \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01}  \\
\end{tabular}}

\raggedleft Exponential moving average alpha = 0.1
\end{table}

==> tables/table17.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!htbp]
\caption{Blockchain SoK and Survey Literature}
\label{tab:17}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lll}

\textbf{Author}                   & \textbf{Category} & \textbf{Title}                                                                    \\ \hline
Almashaqbeh and Solomon (2021) \cite{almashaqbeh_2021_sok}      & Security          & SoK: Privacy-Preserving Computing in the Blockchain Era                           \\ \hline
Bonneau et al. (2015) \cite{bonneau_2015_sok}          & Security          & SoK: Research Perspectives and Challenges for Bitcoin and Cryptocurrencies        \\ \hline
Wang et al. (2021) \cite{wang_2021_sok_b}           & Security          & SoK: Understanding BFT Consensus in the Age of Blockchains                        \\ \hline
Chatzigiannis et al. (2021) \cite{chatzigiannis_2021_sok}    & Security          & SoK: Auditability and Accountability in Distributed Payment Systems               \\ \hline
Eskandari et al. (2019) \cite{eskandari_2019_sok}        & Security          & SoK: Transparent Dishonesty                                                       \\ \hline
Baum et al. (2021) \cite{baum_2021_sok}             & Security          & SoK: Mitigation of Front-running in Decentralized Finance                         \\ \hline
Raikwar et al. (2019) \cite{raikwar_2019_sok}          & Security          & SoK of Used Cryptography in Blockchain                                            \\ \hline
Heimbach et al. (2022) \cite{heimbach_2022_sok}         & Security          & SoK: Preventing Transaction Reordering Manipulations in Decentralized Finance     \\ \hline
Zhou et al. (2022) \cite{zhou_2022_sok}             & Security          & SoK: Decentralized Finance (DeFi) Incidents                                       \\ \hline
Kiayias and Lazos (2022) \cite{kiayias_2022_sok}          & Efficiency        & SoK: Blockchain Governance                                                        \\ \hline
Mccory et al. (2021) \cite{mccorry_2021_sok}          & Efficiency        & SoK: Layer-Two Blockchain Protocols                                               \\ \hline
Wang et al. (2019) \cite{wang_2019_sok}             & Efficiency        & SoK: Sharding on Blockchain                                                       \\ \hline
Zamyatin et al. (2021) \cite{zamyatin_2021_sok}         & Efficiency        & SoK: Communication Across Distributed Ledgers                                     \\ \hline
Wang (2021) \cite{wang_2021_sok}             & Efficiency        & SoK: Exploring Blockchains Interoperability                                       \\ \hline
Bartoletti et al. (2020) \cite{bartoletti_2020_sok}       & Applicability     & SoK: Lending Pools in Decentralized Finance                                       \\ \hline
Werner et al. (2021) \cite{werner_2021_sok}           & Applicability     & SoK: Decentralized Finance (DeFi)                                                 \\ \hline
Xu et al. (2021) \cite{xu_2021_sok}               & Applicability     & SoK: Decentralized Exchanges (DEX) with Automated Market Maker (AMM) Protocols    \\ \hline
Gudgeon et al. (2020) \cite{gudgeon_2020_sok}          & Applicability     & SoK: Layer-Two Blockchain Protocols                                               \\ \hline
Shi et al. (2021) \cite{shi_2021_when}             & Applicability     & When Blockchain Meets Auction Models: A Survey, Some Applications, and Challenges \\ \hline
Abuidris et al. (2019) \cite{abuidris_2019_a}           & Applicability     & A Survey of Blockchain Based on E-voting Systems                                  \\ \hline
Gadekallu et al. (2022) \cite{gadekallu_2022_blockchain} & Applicability     & Blockchain for the Metaverse: A Review                                            \\ \hline
Hassan et al. (2019) \cite{hassan_2019_blockchain}    & Applicability     & Blockchain And The Future of the Internet:A Comprehensive Review                  \\ \hline
Ruoti et al. (2019) \cite{ruoti_2019_sok}            & Applicability     & SoK: Blockchain Technology and Its Potential Use Cases                            \\ \hline
\end{tabular}%
}

{\raggedright \footnotesize \emph{Note: This table summarizes recent blockchain Systematization of Knowledge (SoK) and survey literature by  security, efficiency, and applicability.}\par}
\end{table}

==> tables/table19.tex <==


\begin{table}[!htbp]
	\caption{Autoregression: Sai and Dai Decentralization}
	\label{tab:19}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{llllll}
				\hline
				\multicolumn{3}{c}{{\small\textit{Dependent variable: Decentralization Index}}}\\[-1.8ex]\\
				\hline
				
				\textbf{Lag Period}   & \thead{\makecell{(1) \\ \textbf{Sai}\\ coefficient\\(std.)}} & \thead{\makecell{(2) \\\textbf{Dai}\\ coefficient\\(std.)}}\\
				\\[-1.8ex]\hline
				L1    &   
				\thead{\makecell{$0.6815^{***}$\\(0.039)}}& 	\thead{\makecell{$0.4897^{***}$\\(0.042)}}\\
			
				\hline
			\end{tabular}
		\end{center}
	\footnotesize \bigskip $^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01\\ 
		 This table displays the autoregression results for our dependent variable, the decentralization index. The Newy-West estimator for standard errors was used to adjust for high autocorrelation with day $t-1$.
	\end{minipage}
\end{table}% 

==> tables/table21.tex <==



\begin{table}[!htbp] \centering
  \caption{EIP1559 Regression Discontinuity with Adoption Rate (Dai)}
    \resizebox{0.5\textwidth}{!}{
\begin{tabular}{@{\extracolsep{5pt}}lccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
& \multicolumn{3}{c}{\textit{Dependent variable:} SMA30 Decentralization Index} \
\cr \cline{2-4}
\\[-1.8ex] & (1) & (2) & (3) \\
\hline \\[-1.8ex]
 EIP & 57.686$^{***}$ & 55.970$^{***}$ & 23.983$^{***}$ \\
  & (10.555) & (10.624) & (8.550) \\
 AdoptionRate & 201.287$^{***}$ & 215.055$^{***}$ & 55.530$^{*}$ \\
  & (26.586) & (26.662) & (30.581) \\
 TxTfrValAdjUSD & & -0.000$^{}$ & -0.000$^{}$ \\
  & & (0.000) & (0.000) \\
 TxTfrCnt & & 0.003$^{*}$ & 0.001$^{}$ \\
  & & (0.002) & (0.001) \\
 ROI & & & 8960.151$^{}$ \\
  & & & (5519.973) \\
 VtyDayRet30d & & & 629879.313$^{***}$ \\
  & & & (99323.066) \\
 Intercept & 518.571$^{***}$ & 476.085$^{***}$ & 328.127$^{***}$ \\
  & (6.201) & (30.037) & (30.367) \\
\hline \\[-1.8ex]
 Observations & 33 & 33 & 33 \\
 $R^2$ & 0.903 & 0.919 & 0.968 \\
 Adjusted $R^2$ & 0.897 & 0.907 & 0.961 \\
 Residual Std. Error & 20.567(df = 30) & 19.506(df = 28) & 12.666(df = 26)  \\
 F Statistic & 139.704$^{***}$ (df = 2.0; 30.0) & 78.993$^{***}$ (df = 4.0; 28.0) & 131.641$^{***}$ (df = 6.0; 26.0) \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}}
\end{table}

==> tables/table22.tex <==



\begin{table}[!htbp] \centering
  \caption{EIP1559 Regression Discontinuity with Twice the Bandwidth (Dai)}
  \resizebox{0.5\textwidth}{!}{
\begin{tabular}{@{\extracolsep{5pt}}lccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
& \multicolumn{3}{c}{\textit{Dependent variable:} SMA30 Decentralization Index} \
\cr \cline{2-4}
\\[-1.8ex] & (1) & (2) & (3) \\
\hline \\[-1.8ex]
 EIP & 116.920$^{***}$ & 109.836$^{***}$ & 47.473$^{***}$ \\
  & (12.601) & (12.977) & (11.878) \\
 Day & -7.544$^{***}$ & -7.191$^{***}$ & -3.896$^{***}$ \\
  & (0.824) & (0.827) & (0.705) \\
 EIP\_Day & 9.676$^{***}$ & 9.285$^{***}$ & 6.472$^{***}$ \\
  & (0.874) & (0.890) & (0.711) \\
 TxTfrValAdjUSD & & -0.000$^{**}$ & -0.000$^{**}$ \\
  & & (0.000) & (0.000) \\
 TxTfrCnt & & 0.000$^{}$ & 0.002$^{}$ \\
  & & (0.001) & (0.001) \\
 ROI & & & 3484.025$^{}$ \\
  & & & (5684.337) \\
 VtyDayRet30d & & & 440954.238$^{***}$ \\
  & & & (54503.612) \\
 Intercept & 486.441$^{***}$ & 498.330$^{***}$ & 356.126$^{***}$ \\
  & (10.109) & (25.364) & (25.025) \\
\hline \\[-1.8ex]
 Observations & 66 & 66 & 66 \\
 $R^2$ & 0.836 & 0.847 & 0.928 \\
 Adjusted $R^2$ & 0.828 & 0.834 & 0.920 \\
 Residual Std. Error & 24.522(df = 62) & 24.072(df = 60) & 16.774(df = 58)  \\
 F Statistic & 105.464$^{***}$ (df = 3.0; 62.0) & 66.535$^{***}$ (df = 5.0; 60.0) & 107.244$^{***}$ (df = 7.0; 58.0) \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}}
\end{table}

==> tables/table23.tex <==



\begin{table}[!htbp] \centering
  \caption{EIP1559 Regression Discontinuity with Half the Bandwidth (Dai)}
  \resizebox{0.5\textwidth}{!}{
\begin{tabular}{@{\extracolsep{5pt}}lccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
& \multicolumn{3}{c}{\textit{Dependent variable:} SMA30 Decentralization Index} \
\cr \cline{2-4}
\\[-1.8ex] & (1) & (2) & (3) \\
\hline \\[-1.8ex]
 EIP & 15.536$^{**}$ & 11.740$^{**}$ & 12.388$^{**}$ \\
  & (7.107) & (4.584) & (5.154) \\
 Day & 12.866$^{***}$ & 12.822$^{***}$ & 12.524$^{***}$ \\
  & (1.750) & (1.111) & (1.700) \\
 EIP\_Day & -7.001$^{***}$ & -7.555$^{***}$ & -7.593$^{***}$ \\
  & (1.885) & (1.205) & (1.303) \\
 TxTfrValAdjUSD & & -0.000$^{***}$ & -0.000$^{***}$ \\
  & & (0.000) & (0.000) \\
 TxTfrCnt & & -0.003$^{*}$ & -0.003$^{*}$ \\
  & & (0.001) & (0.001) \\
 ROI & & & -2240.524$^{}$ \\
  & & & (3008.581) \\
 VtyDayRet30d & & & 18084.274$^{}$ \\
  & & & (95192.371) \\
 Intercept & 546.030$^{***}$ & 600.820$^{***}$ & 598.468$^{***}$ \\
  & (5.300) & (21.869) & (42.606) \\
\hline \\[-1.8ex]
 Observations & 17 & 17 & 17 \\
 $R^2$ & 0.980 & 0.993 & 0.994 \\
 Adjusted $R^2$ & 0.975 & 0.990 & 0.989 \\
 Residual Std. Error & 7.322(df = 13) & 4.644(df = 11) & 4.896(df = 9)  \\
 F Statistic & 207.359$^{***}$ (df = 3.0; 13.0) & 313.648$^{***}$ (df = 5.0; 11.0) & 201.685$^{***}$ (df = 7.0; 9.0) \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}}
\end{table}

==> tables/table3.tex <==
\begin{table}[!htbp] \centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{@{\extracolsep{5pt}}lccccccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
& \multicolumn{7}{c}{\textit{Dependent variable: Dai Decentralization Index}} \\

\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) \\
\hline \\[-1.8ex]
 BTC\_Ret & -2896.656$^{}$ & & & & & & \\
  & (1808.711) & & & & & & \\
 BTC\_Ret7 & & -750.178$^{}$ & & & & & \\
  & & (672.075) & & & & & \\
 BTC\_Ret14 & & & -325.353$^{}$ & & & & \\
  & & & (422.519) & & & & \\
 BTC\_Ret21 & & & & 127.183$^{}$ & & & \\
  & & & & (334.516) & & & \\
 BTC\_Ret30 & & & & & 178.575$^{}$ & & \\
  & & & & & (253.038) & & \\
 BTC\_VtyDayRet30d & & & & & & 1588.300$^{}$ & \\
  & & & & & & (2666.581) & \\
 BTC\_PC & & & & & & & 50.838$^{}$ \\
  & & & & & & & (204.327) \\
 const & 1284.587$^{***}$ & 1292.775$^{***}$ & 1290.119$^{***}$ & 1264.126$^{***}$ & 1253.571$^{***}$ & 1213.626$^{***}$ & 1273.973$^{***}$ \\
  & (57.804) & (61.971) & (63.316) & (64.770) & (67.440) & (126.570) & (56.316) \\
\hline \\[-1.8ex]
 Observations & 559 & 559 & 559 & 559 & 559 & 559 & 559 \\
 $R^2$ & 0.014 & 0.007 & 0.003 & 0.001 & 0.002 & 0.001 & 0.000 \\
 Adjusted $R^2$ & 0.012 & 0.005 & 0.001 & -0.001 & 0.000 & -0.001 & -0.001 \\
 Residual Std. Error & 1018.963  & 1022.683  & 1024.682  & 1025.714  & 1024.991  & 1025.637  & 1025.908   \\
 F Statistic & 2.565$^{}$ & 1.246$^{}$ & 0.593$^{}$& 0.145$^{}$ & 0.498$^{}$ & 0.355$^{}$  & 0.062$^{}$\\
\hline
\hline \\[-1.8ex]
\textit{Note:} (df=557) & \multicolumn{7}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}}

\vspace{0.5ex}

{\footnotesize \emph{Note: This table displays the full regression results of Bitcoin market variables on Dai decentralization index as described in our results.} \par}
\end{table}


==> tables/table4.tex <==
\begin{table}[!htbp] \centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{@{\extracolsep{5pt}}lccccccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
& \multicolumn{7}{c}{\textit{Dependent variable:  Sai Decentralization Index}} \\
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) \\
\hline \\[-1.8ex]
 BTC\_Ret & 1998.629$^{}$ & & & & & & \\
  & (1988.974) & & & & & & \\
 BTC\_Ret7 & & 1911.523$^{**}$ & & & & & \\
  & & (798.870) & & & & & \\
 BTC\_Ret14 & & & 1717.610$^{***}$ & & & & \\
  & & & (507.868) & & & & \\
 BTC\_Ret21 & & & & 1653.969$^{***}$ & & & \\
  & & & & (380.851) & & & \\
 BTC\_Ret30 & & & & & 1872.264$^{***}$ & & \\
  & & & & & (291.215) & & \\
 BTC\_VtyDayRet30d & & & & & & 594.051$^{}$ & \\
  & & & & & & (2919.573) & \\
 BTC\_PC & & & & & & & 1206.663$^{***}$ \\
  & & & & & & & (225.768) \\
 const & 1042.219$^{***}$ & 1040.003$^{***}$ & 1030.943$^{***}$ & 1020.407$^{***}$ & 1011.314$^{***}$ & 1019.716$^{***}$ & 1042.491$^{***}$ \\
  & (56.416) & (55.348) & (53.815) & (52.220) & (49.525) & (118.201) & (52.688) \\
\hline \\[-1.8ex]
 Observations & 647 & 647 & 647 & 647 & 647 & 647 & 647 \\
 $R^2$ & 0.005 & 0.033 & 0.058 & 0.086 & 0.145 & 0.000 & 0.120 \\
 Adjusted $R^2$ & 0.003 & 0.032 & 0.057 & 0.084 & 0.144 & -0.001 & 0.119 \\
 Residual Std. Error & 1071.289  & 1055.842  & 1042.084  & 1026.838  & 992.962  & 1073.918  & 1007.404   \\
 F Statistic & 1.010$^{}$   & 5.725$^{**}$   & 11.438$^{***}$   & 18.860$^{***}$   & 41.334$^{***}$   & 0.041$^{}$   & 28.566$^{***}$   \\
\hline
\hline \\[-1.8ex]
\textit{Note:} (df = 645) & \multicolumn{7}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}}

\vspace{0.5ex}

{ \footnotesize \emph{Note: This table displays the full regression results of Bitcoin market variables on Sai decentralization index as described in our results.} \par}
\end{table}


==> tables/table5.tex <==
\begin{table}[!htbp] \centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{@{\extracolsep{5pt}}lccccccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
& \multicolumn{7}{c}{\textit{Dependent variable:Dai Decentralization Index}} \
\cr
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) \\
\hline \\[-1.8ex]
 ETH\_Ret & -1831.393$^{}$ & & & & & & \\
  & (1366.873) & & & & & & \\
 ETH\_Ret7 & & -102.925$^{}$ & & & & & \\
  & & (549.664) & & & & & \\
 ETH\_Ret14 & & & 169.221$^{}$ & & & & \\
  & & & (342.763) & & & & \\
 ETH\_Ret21 & & & & 391.680$^{}$ & & & \\
  & & & & (266.600) & & & \\
 ETH\_Ret30 & & & & & 443.710$^{**}$ & & \\
  & & & & & (191.323) & & \\
 ETH\_VtyDayRet30d & & & & & & -32.986$^{}$ & \\
  & & & & & & (2136.514) & \\
 ETH\_PC & & & & & & & 254.369$^{}$ \\
  & & & & & & & (158.502) \\
 const & 1285.590$^{***}$ & 1278.585$^{***}$ & 1258.554$^{***}$ & 1218.772$^{***}$ & 1181.144$^{***}$ & 1275.678$^{***}$ & 1273.973$^{***}$ \\
  & (58.979) & (63.703) & (65.310) & (68.101) & (69.799) & (133.185) & (55.860) \\
\hline \\[-1.8ex]
 Observations & 559 & 559 & 559 & 559 & 559 & 559 & 559 \\
 $R^2$ & 0.010 & 0.000 & 0.001 & 0.012 & 0.023 & 0.000 & 0.014 \\
 Adjusted $R^2$ & 0.008 & -0.002 & -0.000 & 0.010 & 0.021 & -0.002 & 0.012 \\
 Residual Std. Error & 1020.975  & 1025.956  & 1025.377  & 1020.123  & 1014.436  & 1026.070  & 1018.931   \\
 F Statistic & 1.795$^{}$  & 0.035$^{}$  & 0.244$^{}$  & 2.158$^{}$  & 5.379$^{**}$  & 0.000$^{}$  & 2.575$^{}$  \\
\hline
\hline \\[-1.8ex]
\textit{Note:} (df = 557) & \multicolumn{7}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}}

\vspace{0.5ex}

{ \footnotesize \emph{Note: This table displays the full regression results of Ethereum market variables on the Dai decentralization index as depicted in our results.} \par}
\end{table}


==> tables/table6.tex <==
\begin{table}[!htbp] \centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{@{\extracolsep{5pt}}lccccccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
& \multicolumn{7}{c}{\textit{Dependent variable: Sai Decentralization Index}} \\

\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) \\
\hline \\[-1.8ex]
 ETH\_Ret & 766.402$^{}$ & & & & & & \\
  & (1261.848) & & & & & & \\
 ETH\_Ret7 & & 869.406$^{*}$ & & & & & \\
  & & (520.834) & & & & & \\
 ETH\_Ret14 & & & 784.206$^{***}$ & & & & \\
  & & & (298.941) & & & & \\
 ETH\_Ret21 & & & & 770.518$^{***}$ & & & \\
  & & & & (226.084) & & & \\
 ETH\_Ret30 & & & & & 813.912$^{***}$ & & \\
  & & & & & (182.544) & & \\
 ETH\_VtyDayRet30d & & & & & & -18345.301$^{***}$ & \\
  & & & & & & (3138.375) & \\
 ETH\_PC & & & & & & & 536.188$^{***}$ \\
  & & & & & & & (137.019) \\
 const & 1043.661$^{***}$ & 1051.636$^{***}$ & 1055.066$^{***}$ & 1058.171$^{***}$ & 1069.077$^{***}$ & 1959.454$^{***}$ & 1042.491$^{***}$ \\
  & (56.611) & (56.625) & (56.704) & (56.826) & (57.615) & (183.344) & (55.217) \\
\hline \\[-1.8ex]
 Observations & 647 & 647 & 647 & 647 & 647 & 647 & 647 \\
 $R^2$ & 0.001 & 0.012 & 0.022 & 0.035 & 0.050 & 0.049 & 0.044 \\
 Adjusted $R^2$ & -0.000 & 0.010 & 0.021 & 0.033 & 0.049 & 0.048 & 0.042 \\
 Residual Std. Error & 1073.315  & 1067.556  & 1061.961  & 1055.119  & 1046.736  & 1047.163  & 1050.152   \\
 F Statistic & 0.369$^{}$   & 2.786$^{*}$   & 6.882$^{***}$   & 11.615$^{***}$   & 19.880$^{***}$   & 34.170$^{***}$   & 15.313$^{***}$   \\
\hline
\hline \\[-1.8ex]
\textit{Note:} (df = 645) & \multicolumn{7}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}}

\vspace{0.5ex}

{ \footnotesize \emph{Note: This table displays the full regression results of Ethereum market variables on the Sai decentralization index as depicted in our results.} \par}
\end{table}

